Yet another algorithm to compute the nonlinearity of a Boolean function

We associate to each Boolean function a polynomial whose evaluations represents the distances from all possible Boolean affine functions. Both determining the coefficients of this polynomial from the truth table of the Boolean function and computing its evaluation vector requires a worst-case complexity of $O(n2^n)$ integer operations. This way, with a different approach, we reach the same complexity of established algorithms, such as those based on the fast Walsh transform.

==> secNLwithGBoverF2.tex <==
%
%     \section{Computing the nonlinearity using \Gr\ basis over $\FF_2$}
% % from simonetti
%       \label{secNLwithGBoverF2}
%       \input{tex/secNLwithGBoverF2}  
%
% In this section we show how to use Theorem \ref{gpeso} to compute the nonlinearity of a given Boolean function $f\in \B_n$ ($f$ is understood from now on).\\
% We define an ideal where $\mathfrak{g}_n$ plays the role of a general affine function. A point in its variety corresponds to an affine function with distance from $f$ at most $t-1$.
%
\begin{definition}\label{defIdealF2}
We denote by $J_t^n(f)$ the ideal in $\FF[A]$:
$$
\begin{array}{ll}
J_t^n(f) 
& =
\langle
\{
{\sf m} \big (\mathfrak{g}_n(A,\op_1)+ f(\op_1),\ldots,\mathfrak{g}_n(A,\op_{2^n})+f(\op_{2^n})\big)\mid {\sf m}\in\mathcal{M}_{2^n,t}
\}
\cup 
E[A]
\rangle\\
& = 
\langle\{{\sf m}(\underline{\mathfrak{g}_n}+\ef)\mid {\sf m}\in\mathcal{M}_{2^n,t}\}\cup E[A]\rangle\,.
\end{array}
$$
\end{definition} 
%
\begin{remark}
As $E[A]\subset J_t^n(f)$, $J_t^n(f)$ is zero-dimensional and radical (\cite{CGC-alg-art-seidenberg1}).
\end{remark}
%
\begin{lemma}\label{nf}
For $1\leq t\leq 2^n$ the following statements are equivalent:
\begin{enumerate}
\item $\mathcal{V}(J_t^n(f))\neq \emptyset$,
%\item $\exists u\in S_{\A_n}(f) \textrm{ such that } \w(u)\leq t-1$,
\item $\exists u\in \{\ef+\eg\mid g\in\A_n\} \textrm{ such that } \w(u)\leq t-1$,
\item $\exists \alpha\in\A_n \textrm{ such that } \dist(f,\alpha)\leq t-1$.
\end{enumerate}
\end{lemma}
%
\begin{proof}~\\
(2)$\Leftrightarrow$(3). Obvious.\\
(1)$\Rightarrow$(2). 
Let $V=(\bar{a}_0,\bar{a}_1,\ldots,\bar{a}_n)\in
     \mathcal{V}(J_t^n(f))\subset\FF^{n+1}$ and let $u$ be the element
in $\{\ef+\eg\mid g\in\A_n\}$,
%$S_{\A_n}(f)$, 
then $u=(\mathfrak{g}_n(V,v_1)+f(v_1),\ldots,\mathfrak{g}_n(V,v_{2^n})+f(v_{2^n}))$.
We have that ${\sf m}(u)=0$ for all ${\sf m}\in\mathcal{M}_{2^n,t}$ 
and that $u\in\FF^{2^n}$. So $u\in\mathcal{V}(I_{2^n,t})$ and, 
thanks to Theorem \ref{gpeso}, $u\in Q_{t-1}$, i.e. ${\rm w}(u)\leq t-1$.\\
(2)$\Rightarrow$(1). It can be proved by reversing the above argument.
\end{proof}
%
From Lemma \ref{nf} we immediately have the following theorem.
%
\begin{theorem}\label{Nf}
Let $f\in\B_n$. The nonlinearity $\N(f)$ is the minimum $t$ such that $\mathcal{V}(J_{t+1}^n(f))\neq \emptyset$.
\end{theorem}
%
From this theorem we can derive an algorithm to compute the nonlinearity for a function $f\in\B_n$, by computing any \Gr\ basis of $J_t^n(f)$.
%
\begin{algorithm}[H]
\caption{Basic algorithm to compute the nonlinearity of a Boolean function using \Gr\ basis over $\FF$}
\label{algNLoverF2}
  \begin{algorithmic}[1]
    \REQUIRE{a Boolean function $f$}
    \ENSURE{the nonlinearity of $f$}
    \STATE{$j \leftarrow 1$}
    \WHILE{${\mathcal V}(J_j^n(f)) =\emptyset $} 
      \STATE{$j \leftarrow j+1$} 
    \ENDWHILE
    \RETURN $j-1$
  \end{algorithmic}
\end{algorithm}
%
% \begin{center}
% %\begin{algorithm}
% 
% %{\upshape{
% \newenvironment{tab}[1]%
% {\begin{tabular}{|#1|}\hline}%
% {\hline\end{tabular}}
% 
% 
% \begin{tab}{l}
% 
% %$\vspace{1mm}$
% 
% %\noindent
% 
% 
% $\,\,$ $j=1$\\
% 
% \noindent
% 
% {\bf While} \,\, ${\mathcal V}(J_j^n(f)) =\emptyset $ \,\,\,{\bf do}\\
% 
% $\, \, \, $ $ j:=j+1$;\\
% 
% \noindent
% {\bf Output}  $j-1$\\
% \end{tab}
% \end{center}
%
\begin{remark}
If $f$ is not affine, we can start our check from $J_2^n(f)$.
\end{remark}
%
\begin{example}
Let $f:\FF^3\rightarrow \FF$ be the Boolean function:
$$f(x_1,x_2,x_3)=x_1x_2+x_1x_3+x_2+1\,.$$
We want to compute $\N(f)$ and clearly $f$ is not affine. We compute vector $\ef$ and we take a general affine function $\mathfrak{g}_3$, so that:\\
$\ef=(1,1,0,1,1,0,0,0)$ ,\\
$\underline{\mathfrak{g}_3}=(a_0,a_0+a_1,a_0+a_2,a_0+a_3,a_0+a_1+a_2,a_0+a_1+a_3,a_0+a_2+a_3,a_0+a_1+a_2+a_3).$\\
So $\ef+\underline{\mathfrak{g}_3}=(a_0+1,a_0+a_1+1,a_0+a_2,a_0+a_3+1,a_0+a_1+a_2+1,a_0+a_1+a_3,a_0+a_2+a_3,a_0+a_1+a_2+a_3)=(p_1,p_2,\ldots,p_8)$ .\\
Ideal $J_2^3(f)$ is the ideal generated by
$$J_2^3(f)=\langle\{p_1p_2,p_1p_3,\ldots,p_7p_8\}\cup\{a_0^2+a_0,a_1^2+a_1,a_2^2+a_2,a_3^2+a_3\}\rangle\,.$$
We compute any \Gr\ basis of this ideal and we obtain that it is trivial, so ${\mathcal V}(J_2^3(f)) =\emptyset$ and $\N(f)>1$. Now we have to compute a \Gr\ basis for $J_3^3(f)$. We obtain, using degrevlex ordering with $a_1>a_2>a_3>a_0$, that $G(J_3^3(f))=\{ a_2+a_3+1,a_3^2+a_3,a_1a_3+a_0+1,a_0a_3+a_0+a_3+1, a_1^2+a_1, a_0a_1+a_0+a_1+1, a_0^2+a_0\}$. So, $\N(f)=2$ by Theorem \ref{Nf}. By inspecting $G(J_3^3(f))$, we also obtain all affine functions having distance 2 from $f$:
$$
\begin{array}{cccc}
\alpha_1=1+x_1+x_2, &\; \alpha_2=1+x_2, & \;\alpha_3=1+x_3, & \;\alpha_4=x_1+x_3\,.
\end{array}
$$
\end{example}
%
\begin{example}
Let $f:\FF^5\rightarrow \FF$ be the Boolean function
$$f=x_1x_3x_4x_5  + x_1x_2x_4 +  x_1x_4x_5 + x_2x_3x_4 + x_2x_4x_5 + x_3x_4x_5 + x_4x_5\,.$$
We have that 
$$\ef=(0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,1,0,1,0,0,0,0,1,0,0,0,0,0,0,0,0,1)\,.$$ 
Then we compute $\ef+\underline{\mathfrak{g}_5}$ and we obtain:
$$
\begin{array}{rl}
\ef+\underline{\mathfrak{g}_5} = & (a_0,a_1+a_0,a_2+a_0,a_3+a_0,a_4+a_0,a_5+a_0,a_1+a_2+a_0,\\
& a_1+a_3+a_0,a_1+a_4+a_0,a_1+a_5+a_0,a_2+a_3+a_0, a_2+a_4+a_0,\\
& a_2+a_5+a_0,a_3+a_4+a_0,a_3+a_5+a_0,a_4+a_5+a_0+1,\\
& a_1+a_2+a_3+a_0, a_1+a_2+a_4+a_0+1,a_1+a_2+a_5+a_0,\\
& a_1+a_3+a_4+a_0,a_1+a_3+a_5+a_0, a_1+a_4+a_5+a_0,\\
& a_2+a_3+a_4+a_0+1,a_2+a_3+a_5+a_0,a_2+a_4+a_5+a_0,\\
& a_3+a_4+a_5+a_0,a_1+a_2+a_3+a_4+a_0,a_1+a_2+a_3+a_5+a_0,\\
& a_1+a_2+a_4+a_5+a_0,a_1+a_3+a_4+a_5+a_0,a_2+a_3+a_4+a_5+a_0,\\
& a_1+a_2+a_3+a_4+a_5+a_0+1)= (p_1,p_2,\ldots,p_{32})\,.
\end{array}
$$
As it is obvious that $f$ is not affine, we start from the ideal $J_2^5(f)$, which is generated by
$$J_2^5(f)=\langle\{p_1p_2,p_1p_3,\ldots,p_{31}p_{32}\}\cup\{a_0^2+a_0,a_1^2+a_1,a_2^2+a_2,a_3^2+a_3,a_4^2+a_4,a_5^2+a_5\}\rangle\,.$$
The \Gr\ basis of $J_2^5(f)$ with respect to any monomial order is trivial so we compute a \Gr\ basis of $J_3^5(f)$. We obtain that the \Gr\ basis of $J_t^5(f)$ is trivial with respect to any monomial order for $2\leq t\leq 4$. For $t=5$, we obtain the following \Gr\ basis with respect to the degrevlex order with $a_1>a_2>a_3>a_4>a_5>a_0$:
$$G(J_5^5(f))=\{a_0,a_5,a_4,a_3,a_2,a_1\}\,.$$
Then $\N(f)=4$ and there is only one affine function $\alpha$ which has distance equal to $4$ from $f$: $\alpha=0$.
\end{example}
%

==> secPrelOnGB.tex <==
Here we present the main results from \cite{CGC-cd-prep-maxiladcc}, \cite{CGC-cd-art-ilawcc07}, \cite{CGC-cd-inbook-D1simonetti}. The same techniques are also applied in \cite{CGC-cd-prep-elemanumax} and \cite{CGC-tesi2-guerrini}.
%
\subsection{Polynomials and vector weights}
%
Let $\KK$ be a field and $X=\{x_1,\ldots,x_s\}$ be a set of variables. We denote by $\KK[X]$ the multivariate polynomial ring in the variables X. If $f_1,\ldots,f_N \in \KK[X]$, we denote by $\langle\{f_1,\ldots,f_N\}\rangle$ the ideal in $\KK[X]$ generated by $f_1,\ldots,f_N$. \\
Let $q$ be the power of a prime.
We denote by $E_q[X]=\{x_1^q-x_1,\ldots,x_s^q-x_s\}\,,$ the set of field equations in $\FF_q[X]=\FF_q[x_1,\ldots,x_s]$, where $s\geq 1$ is an integer, understood from now on. We write $E[X]$ when $q=2$.
%
\begin{definition} 
Let $1\leq t \leq s$ and ${\sf m}\in \FF_q [X]$. We say that ${\sf m}$ is 
a {\bf{square free monomial}} of degree $t$ (or a {\bf{simple $t$-monomial}}) if: 
$$
{\sf m} = x_{h_1}\cdots x_{h_t}, \textrm{ where } h_1,\ldots, h_t \in \{1,\ldots,s\} \textrm{ and } h_\ell \neq h_j, \forall \ell\neq j\, ,$$ 
i.e. a monomial in $\FF_q [X]$ such that $\deg_{x_{h_i}}({\sf m})=1$ for any $1\leq i \leq t$. We 
denote by $\mathcal{M}_{s,t}$  the set of all square free monomials of degree $t$ in $\FF_q [X]$.
\end{definition}
%
Let $t\in\NN$, with $1\leq t\leq s$ and let $I_{s,t}\subset\FF_q[X]$  be the following ideal
$$I_{s,t}=\langle\{\sigma_t,\ldots,\sigma_s\}\cup E_q[X]\rangle\,,$$
where $\sigma_i$ are the elementary symmetric functions:
$$
\begin{array}{lcl}
\sigma_1 & = & x_1+x_2+\cdots+x_s,\\
\sigma_2 & = & x_1x_2+x_1x_3+\cdots+x_1x_s+x_2x_3+\cdots+x_{s-1}x_s,\\
 & \cdots\\
 \sigma_{s-1} & = & x_1x_2x_3\cdots x_{s-2}x_{s-1}+\cdots+x_2x_3\cdots x_{s-1}y_s,\\
 \sigma_s & = & x_1x_2\cdots x_{s-1}x_s.
\end{array}
$$
%
We also denote by $I_{s,s+1}$ the ideal $\langle E_q[X] \rangle$.
%
For any $1\leq i\leq s$, let $P_i$ be the set which contains all vectors in $(\FF_q)^n$ of weight $i$, $P_i=\{v\in\FF_q^n\mid \w(v)=i\}$, and let $Q_i$ be the set which contains all vectors of weight up to $i$, $Q_i=\sqcup_{0\leq j\leq i}P_j$ .
%
\begin{theorem}\label{gpeso}
Let $t$ be an integer such that $1\leq t\leq s$. Then the vanishing ideal $\mathcal{I}(Q_t)$ of $Q_{t}$ is
$$\mathcal{I}(Q_t)=I_{s,t+1}\,,$$
and its reduced \Gr\ basis $G$ is
$$
\begin{array}{lcl}
G=E_q[X]\cup\mathcal{M}_{s,t}\,, & \quad & \textrm{for } t\geq 2\,,\\
G=\{x_1,\ldots,x_s\}\,,& \quad & \textrm{for } t=1\,. 
\end{array}
$$
\end{theorem}
%
% Let $I\subset\FF_q[X]$ be an ideal and let $X'$ be a subset of $X$. We denote by $I_{X'}$ the elimination ideal of $I$, i.e. $I_{X'}=I\cap\FF_q[X']$.\\
%
Let $\FF_q[Z]$ be a polynomial ring over $\FF_q$. Let ${\sf m}\in\mathcal{M}_{s,t}$, ${\sf m}=z_{h_1}\cdots z_{h_t}$. For any polynomial vector $W\in(\FF_q[Z])^n$, $W=(W_1,\ldots,W_n)$, we denote by ${\sf m}(W)$ the following polynomial in $\FF_q[Z]$:
$${\sf m}(W)=W_{h_1}\cdot\ldots\cdot W_{h_t}\,.$$
%
\begin{example}
Let $n=s=3,q=2$ and $W=(x_1x_2+x_3,x_2,x_2x_3)\in(\FF[x_1,x_2,x_3])^3$ and ${\sf m}=z_1z_3$. Then
$${\sf m}(W)=(x_1x_2+x_3)(x_2x_3)\,.$$
\end{example}
%
% \subsection{Finding the codewords with weight $\le t$}
% 
% We are now ready to present a general method to find all the codewords of a certain weight less than $t$, using \Gr\ basis.\\
% Suppose we have a code $C$ over $\FF_q$ of length $n$, and suppose that each component can be represented by a polynomial over $\FF_q$ in $s$ variables $X=x_1,\dots,x_s$ (this happens in particular for any systematic, and thus linear, code). We have that:
% $$C=\{(f_1(p_1,\dots,p_s),\dots,f_n(p_1,\dots,p_s)) \mid (p_1,\dots,p_s) \in \FF_q^s\}$$
% Where $f_i(x_1,\dots,x_s) \in \FF_q[X], i=1,\dots,n$.\\
% Then we can define the following ideal:
% $$\W_C^t = \langle E_q[X] \bigcup \{\m(f_1(X),\dots,f_n(X)) \mid \m \in \M_{n,t} \} \rangle$$
% where $E_q[X] = \{x_1^q-x_1,\dots,x_s^q-x_s\}$ are the field equations.\\
% We have the following lemma holding:
% \begin{lemma}
%  Let $C \in \C(n,k,q)$. Let $t \in \NN$ such that $1 \le t \le n$. Then
%  $$\V(\W_C^t) \ne \emptyset \iff \exists c \in C \text{ s.t. } \w(c) \le t-1$$
% \end{lemma}
% Actually, the variety of $\W_C^t$ is the set of points in $\FF^s$ such that evaluated in the defining polynomials $f_i,i=1,\dots,n$ of $C$ give the codewords of $C$ which have weight less than $t$. Clearly this variety is empty if there is no codeword of weight less than $t$.\\
% 
% To find the minimum weight of the code $C$ then we can use the following algorithm:
% \begin{algorithm}[H]
% \caption{Basic algorithm to compute the minimum weight of a code $C$}
% \label{algGeneric}
% \begin{algorithmic}[1]
% \REQUIRE{a $(q,n,k)$-code $C$}
% \ENSURE{the minimum weight of $C$}
% \STATE $j \leftarrow 1$
% \WHILE{$\V(\W_C^j) = \emptyset$} 
%   \STATE{$j \leftarrow j+1$} 
% \ENDWHILE
% \RETURN $j-1$
% \end{algorithmic}
% \end{algorithm}
% 
% We will see in the upcoming chapters how this algorithm has been used to compute the distance of a systematic code and the nonlinearity of a boolean function.
